Magnetized Rotating Isothermal Winds

We consider the general problem of a Parker-type non-relativistic isothermal wind from a rotating and magnetic star. Using the magnetohydrodynamics (MHD) code athena++, we construct an array of simulations in the stellar rotation rate $\Omega_\ast$ and the isothermal sound speed $c_T$, and calculate the mass, angular momentum, and energy loss rates across this parameter space. We also briefly consider the three dimensional case, with misaligned magnetic and rotation axes. We discuss applications of our results to the spindown of normal stars, highly-irradiated exoplanets, and to nascent highly-magnetic and rapidly-rotating neutron stars born in massive star core collapse.8

==> Tables/array-compl-9-c-new.tex <==
\begin{tabular}{ccccccc}
\hline$\xi_T$ & $\xi_\varOmega$ & $\log_{10}\dot{M}$ & $\log_{10}\dot{J}$ & $\log_{10}\dot{E}$ & $\log_{10}\tau_J$ & $\Phi/\Phi_0$\\
\hline\hline
%9
0.187 & 0.153 & -3.0154 & -2.2921 & -1.9778 & 5.2397 & 0.6572\\
      & 0.126 & -3.1818 & -2.3518 & -2.1266 & 5.2994 & 0.6388\\
      & 0.103 & -3.3311 & -2.4062 & -2.2582 & 5.3538 & 0.6118\\
      & 0.085 & -3.4549 & -2.4463 & -2.3643 & 5.3939 & 0.5861\\
      & 0.069 & -3.5556 & -2.4601 & -2.4526 & 5.4077 & 0.5830\\
      & 0.057 & -3.6400 & -2.4775 & -2.5246 & 5.4251 & 0.5683\\
      & 0.047 & -3.7053 & -2.4855 & -2.5799 & 5.4332 & 0.5626\\
      & 0.038 & -3.7546 & -2.4819 & -2.6212 & 5.4295 & 0.5644\\
      & 0.031 & -3.7920 & -2.4811 & -2.6521 & 5.4287 & 0.5612\\
      & 0.026 & -3.8195 & -2.4851 & -2.6745 & 5.4328 & 0.5545\\
      & 0.021 & -3.8392 & -2.4899 & -2.6903 & 5.4375 & 0.5473\\
      & 0.017 & -3.8529 & -2.4913 & -2.7013 & 5.4390 & 0.5443\\
%a
0.179 
%~ & 0.278 & -2.4555 & -1.9830 & -1.5104 & 4.9306 & 0.8906\\
      %~ & 0.228 & -2.7401 & -0.5064 & 1.2505 & 3.4540 & 7.7365\\
      %~ & 0.187 & -2.9683 & -2.1018 & -1.6299 & 5.0494 & 1.7042\\
      & 0.153 & -3.2555 & -2.4330 & -2.2185 & 5.3806 & 0.6145\\
      & 0.126 & -3.4635 & -2.5247 & -2.4065 & 5.4723 & 0.5729\\
      & 0.103 & -3.6463 & -2.5974 & -2.5693 & 5.5450 & 0.5380\\
      & 0.085 & -3.8020 & -2.6629 & -2.7023 & 5.6105 & 0.4982\\
      & 0.069 & -3.9330 & -2.7091 & -2.8149 & 5.6567 & 0.4711\\
      & 0.057 & -4.0366 & -2.7324 & -2.9030 & 5.6800 & 0.4566\\
      & 0.047 & -4.1173 & -2.7413 & -2.9706 & 5.6889 & 0.4481\\
      & 0.038 & -4.1793 & -2.7352 & -3.0222 & 5.6828 & 0.4491\\
      & 0.031 & -4.2283 & -2.7409 & -3.0617 & 5.6885 & 0.4428\\
      & 0.026 & -4.2649 & -2.7511 & -3.0905 & 5.6987 & 0.4333\\
      & 0.021 & -4.2909 & -2.7465 & -3.1110 & 5.6941 & 0.4321\\
      & 0.017 & -4.3098 & -2.7496 & -3.1258 & 5.6973 & 0.4284\\
%b
0.172 
%~ & 0.278 & -2.5697 & -2.0533 & -1.6274 & 5.0009 & 0.8776\\
      %~ & 0.187 & -3.1699 & -2.3306 & -2.2086 & 5.2782 & 0.7695\\
      & 0.153 & -3.4601 & -2.4840 & -2.4768 & 5.4316 & 0.6772\\
      & 0.126 & -3.7759 & -2.7147 & -2.7369 & 5.6623 & 0.5047\\
      & 0.103 & -3.9985 & -2.8054 & -2.9390 & 5.7531 & 0.4628\\
      & 0.085 & -4.1891 & -2.8879 & -3.1026 & 5.8356 & 0.4246\\
      & 0.069 & -4.3525 & -2.9470 & -3.2409 & 5.8946 & 0.3903\\
      & 0.057 & -4.4890 & -3.0051 & -3.3516 & 5.9527 & 0.3632\\
      & 0.047 & -4.5967 & -3.0478 & -3.4369 & 5.9954 & 0.3376\\
      & 0.038 & -4.6756 & -3.0705 & -3.4983 & 6.0181 & 0.3287\\
      & 0.031 & -4.7373 & -3.0891 & -3.5456 & 6.0367 & 0.3168\\
      & 0.026 & -4.7788 & -3.0734 & -3.5777 & 6.0210 & 0.3192\\
      & 0.021 & -4.8118 & -3.0704 & -3.6023 & 6.0180 & 0.3149\\
      & 0.017 & -4.8377 & -3.0876 & -3.6213 & 6.0352 & 0.3044\\
%c
0.164 
%~ & 0.228 & -3.0905 & -2.2984 & -1.8560 & 5.2460 & 1.4012\\
      %~ & 0.187 & -3.4114 & -2.4577 & -2.5336 & 5.4053 & 0.7450\\
      & 0.126 & -4.1229 & -2.8974 & -3.1711 & 5.8450 & 0.4630\\
      & 0.103 & -4.3962 & -3.0088 & -3.4336 & 5.9564 & 0.4180\\
      & 0.085 & -4.6305 & -3.1035 & -3.6377 & 6.0511 & 0.3761\\
      & 0.069 & -4.8374 & -3.1924 & -3.8040 & 6.1400 & 0.3436\\
      & 0.057 & -5.0101 & -3.2651 & -3.9304 & 6.2127 & 0.3119\\
      & 0.047 & -5.1437 & -3.3119 & -4.0220 & 6.2595 & 0.2863\\
      & 0.038 & -5.2491 & -3.3484 & -4.0912 & 6.2960 & 0.2669\\
      & 0.031 & -5.3365 & -3.3888 & -4.1479 & 6.3364 & 0.2502\\
      & 0.026 & -5.3972 & -3.4134 & -4.1853 & 6.3611 & 0.2401\\
      & 0.021 & -5.4495 & -3.4452 & -4.2195 & 6.3928 & 0.2263\\
      & 0.017 & -5.4668 & -3.4253 & -4.2253 & 6.3729 & 0.2259\\
\hline\end{tabular}


==> Tables/array-compl-9-c.tex <==
\begin{tabular}{ccccccc}
\hline$\xi_T$ & $\xi_\varOmega$ & $\log_{10}\dot{M}$ & $\log_{10}\dot{J}$ & $\log_{10}\dot{E}$ & $\log_{10}\tau_J$ & $\Phi/\Phi_0$\\
\hline\hline
%9
0.187 & 0.153 & -3.0154 & -2.2921 & -1.9778 & 5.2397 & 0.6572\\
      & 0.126 & -3.1818 & -2.3518 & -2.1266 & 5.2994 & 0.6388\\
      & 0.103 & -3.3311 & -2.4062 & -2.2582 & 5.3538 & 0.6118\\
      & 0.085 & -3.4549 & -2.4463 & -2.3643 & 5.3939 & 0.5861\\
      & 0.069 & -3.5556 & -2.4601 & -2.4526 & 5.4077 & 0.5830\\
      & 0.057 & -3.6400 & -2.4775 & -2.5246 & 5.4251 & 0.5683\\
      & 0.047 & -3.7053 & -2.4855 & -2.5799 & 5.4332 & 0.5626\\
      & 0.038 & -3.7546 & -2.4819 & -2.6212 & 5.4295 & 0.5644\\
      & 0.031 & -3.7920 & -2.4811 & -2.6521 & 5.4287 & 0.5612\\
      & 0.026 & -3.8195 & -2.4851 & -2.6745 & 5.4328 & 0.5545\\
      & 0.021 & -3.8392 & -2.4899 & -2.6903 & 5.4375 & 0.5473\\
      & 0.017 & -3.8529 & -2.4913 & -2.7013 & 5.4390 & 0.5443\\
%a
0.179 & 0.278 & -2.4555 & -1.9830 & -1.5104 & 4.9306 & 0.8906\\
      & 0.228 & -2.7401 & -0.5064 & 1.2505 & 3.4540 & 7.7365\\
      & 0.187 & -2.9683 & -2.1018 & -1.6299 & 5.0494 & 1.7042\\
      & 0.153 & -3.2555 & -2.4330 & -2.2185 & 5.3806 & 0.6145\\
      & 0.126 & -3.4635 & -2.5247 & -2.4065 & 5.4723 & 0.5729\\
      & 0.103 & -3.6463 & -2.5974 & -2.5693 & 5.5450 & 0.5380\\
      & 0.085 & -3.8020 & -2.6629 & -2.7023 & 5.6105 & 0.4982\\
      & 0.069 & -3.9330 & -2.7091 & -2.8149 & 5.6567 & 0.4711\\
      & 0.057 & -4.0366 & -2.7324 & -2.9030 & 5.6800 & 0.4566\\
      & 0.047 & -4.1173 & -2.7413 & -2.9706 & 5.6889 & 0.4481\\
      & 0.038 & -4.1793 & -2.7352 & -3.0222 & 5.6828 & 0.4491\\
      & 0.031 & -4.2283 & -2.7409 & -3.0617 & 5.6885 & 0.4428\\
      & 0.026 & -4.2649 & -2.7511 & -3.0905 & 5.6987 & 0.4333\\
      & 0.021 & -4.2909 & -2.7465 & -3.1110 & 5.6941 & 0.4321\\
      & 0.017 & -4.3098 & -2.7496 & -3.1258 & 5.6973 & 0.4284\\
%b
0.172 & 0.278 & -2.5697 & -2.0533 & -1.6274 & 5.0009 & 0.8776\\
      & 0.187 & -3.1699 & -2.3306 & -2.2086 & 5.2782 & 0.7695\\
      & 0.153 & -3.4601 & -2.4840 & -2.4768 & 5.4316 & 0.6772\\
      & 0.126 & -3.7759 & -2.7147 & -2.7369 & 5.6623 & 0.5047\\
      & 0.103 & -3.9985 & -2.8054 & -2.9390 & 5.7531 & 0.4628\\
      & 0.085 & -4.1891 & -2.8879 & -3.1026 & 5.8356 & 0.4246\\
      & 0.069 & -4.3525 & -2.9470 & -3.2409 & 5.8946 & 0.3903\\
      & 0.057 & -4.4890 & -3.0051 & -3.3516 & 5.9527 & 0.3632\\
      & 0.047 & -4.5967 & -3.0478 & -3.4369 & 5.9954 & 0.3376\\
      & 0.038 & -4.6756 & -3.0705 & -3.4983 & 6.0181 & 0.3287\\
      & 0.031 & -4.7373 & -3.0891 & -3.5456 & 6.0367 & 0.3168\\
      & 0.026 & -4.7788 & -3.0734 & -3.5777 & 6.0210 & 0.3192\\
      & 0.021 & -4.8118 & -3.0704 & -3.6023 & 6.0180 & 0.3149\\
      & 0.017 & -4.8377 & -3.0876 & -3.6213 & 6.0352 & 0.3044\\
%c
0.164 & 0.228 & -3.0905 & -2.2984 & -1.8560 & 5.2460 & 1.4012\\
      & 0.187 & -3.4114 & -2.4577 & -2.5336 & 5.4053 & 0.7450\\
      & 0.126 & -4.1229 & -2.8974 & -3.1711 & 5.8450 & 0.4630\\
      & 0.103 & -4.3962 & -3.0088 & -3.4336 & 5.9564 & 0.4180\\
      & 0.085 & -4.6305 & -3.1035 & -3.6377 & 6.0511 & 0.3761\\
      & 0.069 & -4.8374 & -3.1924 & -3.8040 & 6.1400 & 0.3436\\
      & 0.057 & -5.0101 & -3.2651 & -3.9304 & 6.2127 & 0.3119\\
      & 0.047 & -5.1437 & -3.3119 & -4.0220 & 6.2595 & 0.2863\\
      & 0.038 & -5.2491 & -3.3484 & -4.0912 & 6.2960 & 0.2669\\
      & 0.031 & -5.3365 & -3.3888 & -4.1479 & 6.3364 & 0.2502\\
      & 0.026 & -5.3972 & -3.4134 & -4.1853 & 6.3611 & 0.2401\\
      & 0.021 & -5.4495 & -3.4452 & -4.2195 & 6.3928 & 0.2263\\
      & 0.017 & -5.4668 & -3.4253 & -4.2253 & 6.3729 & 0.2259\\
\hline\end{tabular}


==> Tables/array-full-1.tex <==
0.247 & 0.278 & -1.4008 & -1.3939 & -0.5419 & 4.3416 & 0.9758\\
 & 0.228 & -1.4700 & -1.4368 & -0.5965 & 4.3845 & 0.9564\\
 & 0.187 & -1.5273 & -1.4703 & -0.6427 & 4.4179 & 0.9481\\
 & 0.153 & -1.5718 & -1.4946 & -0.6789 & 4.4423 & 0.9523\\
 & 0.126 & -1.6050 & -1.5080 & -0.7060 & 4.4556 & 0.9616\\
 & 0.103 & -1.6283 & -1.5058 & -0.7252 & 4.4534 & 0.9898\\
 & 0.085 & -1.6465 & -1.5117 & -0.7402 & 4.4593 & 0.9968\\
 & 0.069 & -1.6598 & -1.5182 & -0.7510 & 4.4658 & 0.9967\\
 & 0.057 & -1.6690 & -1.5224 & -0.7586 & 4.4700 & 0.9979\\
 & 0.047 & -1.6754 & -1.5257 & -0.7639 & 4.4733 & 0.9989\\
 & 0.038 & -1.6797 & -1.5275 & -0.7674 & 4.4751 & 0.9992\\
 & 0.031 & -1.6827 & -1.5284 & -0.7699 & 4.4761 & 0.9990\\
 & 0.026 & -1.6847 & -1.5291 & -0.7716 & 4.4767 & 0.9994\\
 & 0.021 & -1.6861 & -1.5295 & -0.7727 & 4.4771 & 0.9996\\
 & 0.017 & -1.6870 & -1.5297 & -0.7734 & 4.4774 & 0.9998\\


==> Tables/array-full-2.tex <==
0.240 & 0.278 & -1.4983 & -1.4626 & -0.6136 & 4.4103 & 0.9370\\
 & 0.228 & -1.5800 & -1.4863 & -0.6872 & 4.4339 & 0.9196\\
 & 0.187 & -1.6540 & -1.5326 & -0.7480 & 4.4802 & 0.9100\\
 & 0.153 & -1.7108 & -1.5655 & -0.7951 & 4.5131 & 0.9121\\
 & 0.126 & -1.7530 & -1.5815 & -0.8303 & 4.5291 & 0.9244\\
 & 0.103 & -1.7832 & -1.5806 & -0.8556 & 4.5282 & 0.9534\\
 & 0.085 & -1.8060 & -1.5785 & -0.8746 & 4.5261 & 0.9747\\
 & 0.069 & -1.8231 & -1.5780 & -0.8889 & 4.5256 & 0.9870\\
 & 0.057 & -1.8355 & -1.5783 & -0.8993 & 4.5259 & 0.9949\\
 & 0.047 & -1.8443 & -1.5801 & -0.9066 & 4.5277 & 0.9965\\
 & 0.038 & -1.8505 & -1.5818 & -0.9117 & 4.5295 & 0.9974\\
 & 0.031 & -1.8547 & -1.5828 & -0.9152 & 4.5304 & 0.9984\\
 & 0.026 & -1.8576 & -1.5834 & -0.9176 & 4.5311 & 0.9986\\
 & 0.021 & -1.8595 & -1.5838 & -0.9193 & 4.5314 & 0.9989\\
 & 0.017 & -1.8608 & -1.5840 & -0.9204 & 4.5316 & 0.9990\\


==> Tables/array-full-3.tex <==
0.232 & 0.278 & -1.5902 & -1.4833 & -0.6932 & 4.4309 & 0.9121\\
 & 0.228 & -1.7000 & -1.5472 & -0.7876 & 4.4948 & 0.8818\\
 & 0.187 & -1.7916 & -1.6074 & -0.8643 & 4.5550 & 0.8710\\
 & 0.153 & -1.8624 & -1.6457 & -0.9240 & 4.5933 & 0.8764\\
 & 0.126 & -1.9135 & -1.6600 & -0.9673 & 4.6076 & 0.8956\\
 & 0.103 & -1.9526 & -1.6640 & -1.0004 & 4.6117 & 0.9165\\
 & 0.085 & -1.9826 & -1.6660 & -1.0258 & 4.6136 & 0.9314\\
 & 0.069 & -2.0048 & -1.6641 & -1.0445 & 4.6118 & 0.9460\\
 & 0.057 & -2.0210 & -1.6618 & -1.0583 & 4.6094 & 0.9561\\
 & 0.047 & -2.0327 & -1.6589 & -1.0681 & 4.6065 & 0.9656\\
 & 0.038 & -2.0410 & -1.6571 & -1.0751 & 4.6047 & 0.9712\\
 & 0.031 & -2.0467 & -1.6550 & -1.0799 & 4.6027 & 0.9762\\
 & 0.026 & -2.0507 & -1.6532 & -1.0832 & 4.6008 & 0.9806\\
 & 0.021 & -2.0534 & -1.6509 & -1.0855 & 4.5986 & 0.9849\\
 & 0.017 & -2.0552 & -1.6497 & -1.0870 & 4.5973 & 0.9879\\


==> Tables/array-full-4.tex <==
0.225 & 0.278 & -1.6915 & -1.5248 & -0.7819 & 4.4724 & 0.8616\\
 & 0.228 & -1.8270 & -1.6172 & -0.8957 & 4.5648 & 0.8390\\
 & 0.187 & -1.9400 & -1.6916 & -0.9917 & 4.6392 & 0.8315\\
 & 0.153 & -2.0249 & -1.7334 & -1.0643 & 4.6810 & 0.8401\\
 & 0.126 & -2.0886 & -1.7532 & -1.1190 & 4.7008 & 0.8514\\
 & 0.103 & -2.1385 & -1.7625 & -1.1617 & 4.7101 & 0.8666\\
 & 0.085 & -2.1766 & -1.7638 & -1.1943 & 4.7114 & 0.8814\\
 & 0.069 & -2.2056 & -1.7640 & -1.2191 & 4.7116 & 0.8922\\
 & 0.057 & -2.2274 & -1.7657 & -1.2376 & 4.7133 & 0.8970\\
 & 0.047 & -2.2431 & -1.7664 & -1.2509 & 4.7140 & 0.8995\\
 & 0.038 & -2.2541 & -1.7655 & -1.2603 & 4.7131 & 0.9034\\
 & 0.031 & -2.2618 & -1.7641 & -1.2668 & 4.7117 & 0.9070\\
 & 0.026 & -2.2671 & -1.7629 & -1.2713 & 4.7105 & 0.9098\\
 & 0.021 & -2.2708 & -1.7619 & -1.2744 & 4.7095 & 0.9118\\
 & 0.017 & -2.2733 & -1.7612 & -1.2765 & 4.7088 & 0.9132\\


==> Tables/array-full-5.tex <==
0.217 & 0.278 & -1.8019 & -1.5857 & -0.8756 & 4.5333 & 0.8184\\
 & 0.228 & -1.9627 & -1.6959 & -1.0129 & 4.6435 & 0.8015\\
 & 0.187 & -2.0957 & -1.7772 & -1.1278 & 4.7248 & 0.7998\\
 & 0.153 & -2.1983 & -1.8289 & -1.2165 & 4.7765 & 0.7998\\
 & 0.126 & -2.2778 & -1.8548 & -1.2853 & 4.8024 & 0.8083\\
 & 0.103 & -2.3408 & -1.8711 & -1.3398 & 4.8187 & 0.8167\\
 & 0.085 & -2.3897 & -1.8782 & -1.3819 & 4.8258 & 0.8228\\
 & 0.069 & -2.4280 & -1.8874 & -1.4148 & 4.8350 & 0.8186\\
 & 0.057 & -2.4564 & -1.8935 & -1.4392 & 4.8411 & 0.8144\\
 & 0.047 & -2.4769 & -1.8957 & -1.4567 & 4.8433 & 0.8135\\
 & 0.038 & -2.4916 & -1.8979 & -1.4692 & 4.8455 & 0.8111\\
 & 0.031 & -2.5020 & -1.8992 & -1.4780 & 4.8468 & 0.8094\\
 & 0.026 & -2.5091 & -1.9003 & -1.4841 & 4.8479 & 0.8078\\
 & 0.021 & -2.5140 & -1.9011 & -1.4883 & 4.8487 & 0.8065\\
 & 0.017 & -2.5174 & -1.9017 & -1.4912 & 4.8493 & 0.8055\\


==> Tables/array-full-6.tex <==
0.210 & 0.278 & -1.9209 & -1.6556 & -0.9788 & 4.6032 & 0.7845\\
 & 0.228 & -2.1118 & -1.7905 & -1.1446 & 4.7382 & 0.7693\\
 & 0.187 & -2.2638 & -1.8780 & -1.2768 & 4.8256 & 0.7589\\
 & 0.153 & -2.3850 & -1.9346 & -1.3829 & 4.8822 & 0.7644\\
 & 0.126 & -2.4820 & -1.9698 & -1.4677 & 4.9175 & 0.7608\\
 & 0.103 & -2.5603 & -1.9915 & -1.5359 & 4.9391 & 0.7628\\
 & 0.085 & -2.6228 & -2.0049 & -1.5902 & 4.9525 & 0.7604\\
 & 0.069 & -2.6722 & -2.0170 & -1.6328 & 4.9646 & 0.7526\\
 & 0.057 & -2.7097 & -2.0261 & -1.6651 & 4.9737 & 0.7448\\
 & 0.047 & -2.7371 & -2.0304 & -1.6886 & 4.9780 & 0.7402\\
 & 0.038 & -2.7571 & -2.0356 & -1.7057 & 4.9832 & 0.7336\\
 & 0.031 & -2.7713 & -2.0403 & -1.7178 & 4.9879 & 0.7274\\
 & 0.026 & -2.7812 & -2.0460 & -1.7263 & 4.9936 & 0.7200\\
 & 0.021 & -2.7880 & -2.0510 & -1.7321 & 4.9986 & 0.7135\\
 & 0.017 & -2.7927 & -2.0549 & -1.7360 & 5.0025 & 0.7086\\


==> Tables/array-full-7.tex <==
0.202 & 0.187 & -2.4319 & -1.9712 & -1.4350 & 4.9188 & 0.7389\\
 & 0.153 & -2.5774 & -2.0382 & -1.5623 & 4.9858 & 0.7378\\
 & 0.126 & -2.7009 & -2.0912 & -1.6698 & 5.0388 & 0.7275\\
 & 0.103 & -2.7978 & -2.1175 & -1.7541 & 5.0651 & 0.7230\\
 & 0.085 & -2.8746 & -2.1320 & -1.8193 & 5.0796 & 0.7108\\
 & 0.069 & -2.9378 & -2.1426 & -1.8741 & 5.0903 & 0.7066\\
 & 0.057 & -2.9873 & -2.1503 & -1.9167 & 5.0979 & 0.6994\\
 & 0.047 & -3.0249 & -2.1568 & -1.9489 & 5.1044 & 0.6940\\
 & 0.038 & -3.0522 & -2.1583 & -1.9722 & 5.1059 & 0.6920\\
 & 0.031 & -3.0720 & -2.1607 & -1.9890 & 5.1083 & 0.6882\\
 & 0.026 & -3.0861 & -2.1631 & -2.0009 & 5.1107 & 0.6841\\
 & 0.021 & -3.0958 & -2.1643 & -2.0092 & 5.1119 & 0.6818\\
 & 0.017 & -3.1025 & -2.1635 & -2.0148 & 5.1111 & 0.6821\\


==> Tables/array-full-8.tex <==
0.194 & 0.153 & -2.7913 & -2.1642 & -1.7616 & 5.1118 & 0.6910\\
 & 0.126 & -2.9336 & -2.2175 & -1.8871 & 5.1651 & 0.6835\\
 & 0.103 & -3.0529 & -2.2534 & -1.9917 & 5.2010 & 0.6694\\
 & 0.085 & -3.1531 & -2.2865 & -2.0769 & 5.2341 & 0.6424\\
 & 0.069 & -3.2334 & -2.3004 & -2.1469 & 5.2480 & 0.6361\\
 & 0.057 & -3.2967 & -2.3045 & -2.2016 & 5.2521 & 0.6357\\
 & 0.047 & -3.3459 & -2.3070 & -2.2437 & 5.2547 & 0.6337\\
 & 0.038 & -3.3829 & -2.3036 & -2.2751 & 5.2513 & 0.6362\\
 & 0.031 & -3.4101 & -2.3014 & -2.2980 & 5.2490 & 0.6381\\
 & 0.026 & -3.4297 & -2.2979 & -2.3144 & 5.2455 & 0.6394\\
 & 0.021 & -3.4436 & -2.2960 & -2.3260 & 5.2436 & 0.6410\\
 & 0.017 & -3.4534 & -2.2912 & -2.3341 & 5.2388 & 0.6428\\


==> Tables/array-full-9.tex <==
0.187 & 0.153 & -3.0154 & -2.2921 & -1.9778 & 5.2397 & 0.6572\\
 & 0.126 & -3.1818 & -2.3518 & -2.1266 & 5.2994 & 0.6388\\
 & 0.103 & -3.3311 & -2.4062 & -2.2582 & 5.3538 & 0.6118\\
 & 0.085 & -3.4549 & -2.4463 & -2.3643 & 5.3939 & 0.5861\\
 & 0.069 & -3.5556 & -2.4601 & -2.4526 & 5.4077 & 0.5830\\
 & 0.057 & -3.6400 & -2.4775 & -2.5246 & 5.4251 & 0.5683\\
 & 0.047 & -3.7053 & -2.4855 & -2.5799 & 5.4332 & 0.5626\\
 & 0.038 & -3.7546 & -2.4819 & -2.6212 & 5.4295 & 0.5644\\
 & 0.031 & -3.7920 & -2.4811 & -2.6521 & 5.4287 & 0.5612\\
 & 0.026 & -3.8195 & -2.4851 & -2.6745 & 5.4328 & 0.5545\\
 & 0.021 & -3.8392 & -2.4899 & -2.6903 & 5.4375 & 0.5473\\
 & 0.017 & -3.8529 & -2.4913 & -2.7013 & 5.4390 & 0.5443\\


==> Tables/array-full-a.tex <==
0.179 & 0.278 & -2.4555 & -1.9830 & -1.5104 & 4.9306 & 0.8906\\
 & 0.228 & -2.7401 & -0.5064 & 1.2505 & 3.4540 & 7.7365\\
 & 0.187 & -2.9683 & -2.1018 & -1.6299 & 5.0494 & 1.7042\\
 & 0.153 & -3.2555 & -2.4330 & -2.2185 & 5.3806 & 0.6145\\
 & 0.126 & -3.4635 & -2.5247 & -2.4065 & 5.4723 & 0.5729\\
 & 0.103 & -3.6463 & -2.5974 & -2.5693 & 5.5450 & 0.5380\\
 & 0.085 & -3.8020 & -2.6629 & -2.7023 & 5.6105 & 0.4982\\
 & 0.069 & -3.9330 & -2.7091 & -2.8149 & 5.6567 & 0.4711\\
 & 0.057 & -4.0366 & -2.7324 & -2.9030 & 5.6800 & 0.4566\\
 & 0.047 & -4.1173 & -2.7413 & -2.9706 & 5.6889 & 0.4481\\
 & 0.038 & -4.1793 & -2.7352 & -3.0222 & 5.6828 & 0.4491\\
 & 0.031 & -4.2283 & -2.7409 & -3.0617 & 5.6885 & 0.4428\\
 & 0.026 & -4.2649 & -2.7511 & -3.0905 & 5.6987 & 0.4333\\
 & 0.021 & -4.2909 & -2.7465 & -3.1110 & 5.6941 & 0.4321\\
 & 0.017 & -4.3098 & -2.7496 & -3.1258 & 5.6973 & 0.4284\\


==> Tables/array-full-b.tex <==
0.172 & 0.278 & -2.5697 & -2.0533 & -1.6274 & 5.0009 & 0.8776\\
 & 0.187 & -3.1699 & -2.3306 & -2.2086 & 5.2782 & 0.7695\\
 & 0.153 & -3.4601 & -2.4840 & -2.4768 & 5.4316 & 0.6772\\
 & 0.126 & -3.7759 & -2.7147 & -2.7369 & 5.6623 & 0.5047\\
 & 0.103 & -3.9985 & -2.8054 & -2.9390 & 5.7531 & 0.4628\\
 & 0.085 & -4.1891 & -2.8879 & -3.1026 & 5.8356 & 0.4246\\
 & 0.069 & -4.3525 & -2.9470 & -3.2409 & 5.8946 & 0.3903\\
 & 0.057 & -4.4890 & -3.0051 & -3.3516 & 5.9527 & 0.3632\\
 & 0.047 & -4.5967 & -3.0478 & -3.4369 & 5.9954 & 0.3376\\
 & 0.038 & -4.6756 & -3.0705 & -3.4983 & 6.0181 & 0.3287\\
 & 0.031 & -4.7373 & -3.0891 & -3.5456 & 6.0367 & 0.3168\\
 & 0.026 & -4.7788 & -3.0734 & -3.5777 & 6.0210 & 0.3192\\
 & 0.021 & -4.8118 & -3.0704 & -3.6023 & 6.0180 & 0.3149\\
 & 0.017 & -4.8377 & -3.0876 & -3.6213 & 6.0352 & 0.3044\\


==> Tables/array-full-c.tex <==
0.164 & 0.228 & -3.0905 & -2.2984 & -1.8560 & 5.2460 & 1.4012\\
 & 0.187 & -3.4114 & -2.4577 & -2.5336 & 5.4053 & 0.7450\\
 & 0.126 & -4.1229 & -2.8974 & -3.1711 & 5.8450 & 0.4630\\
 & 0.103 & -4.3962 & -3.0088 & -3.4336 & 5.9564 & 0.4180\\
 & 0.085 & -4.6305 & -3.1035 & -3.6377 & 6.0511 & 0.3761\\
 & 0.069 & -4.8374 & -3.1924 & -3.8040 & 6.1400 & 0.3436\\
 & 0.057 & -5.0101 & -3.2651 & -3.9304 & 6.2127 & 0.3119\\
 & 0.047 & -5.1437 & -3.3119 & -4.0220 & 6.2595 & 0.2863\\
 & 0.038 & -5.2491 & -3.3484 & -4.0912 & 6.2960 & 0.2669\\
 & 0.031 & -5.3365 & -3.3888 & -4.1479 & 6.3364 & 0.2502\\
 & 0.026 & -5.3972 & -3.4134 & -4.1853 & 6.3611 & 0.2401\\
 & 0.021 & -5.4495 & -3.4452 & -4.2195 & 6.3928 & 0.2263\\
 & 0.017 & -5.4668 & -3.4253 & -4.2253 & 6.3729 & 0.2259\\


==> Tables/array-full-foot.tex <==
\hline\end{tabular}


==> Tables/array-full-head.tex <==
\begin{tabular}{ccccccc}
\hline$\xi_T$ & $\xi_\varOmega$ & $\log_{10}\dot{M}$ & $\log_{10}\dot{J}$ & $\log_{10}\dot{E}$ & $\log_{10}\tau_J$ & $\Phi/\Phi_0$\\
\hline\hline

